SafeChat: A Framework for Building Trustworthy Collaborative Assistants and a Case Study of its Usefulness

Collaborative assistants, or chatbots, are data-driven decision support systems that enable natural interaction for task completion. While they can meet critical needs in modern society, concerns about their reliability and trustworthiness persist. In particular, Large Language Model (LLM)-based chatbots like ChatGPT, Gemini, and DeepSeek are becoming more accessible. However, such chatbots have limitations, including their inability to explain response generation, the risk of generating problematic content, the lack of standardized testing for reliability, and the need for deep AI expertise and extended development times. These issues make chatbots unsuitable for trust-sensitive applications like elections or healthcare. To address these concerns, we introduce SafeChat, a general architecture for building safe and trustworthy chatbots, with a focus on information retrieval use cases. Key features of SafeChat include: (a) safety, with a domain-agnostic design where responses are grounded and traceable to approved sources (provenance), and 'do-not-respond' strategies to prevent harmful answers; (b) usability, with automatic extractive summarization of long responses, traceable to their sources, and automated trust assessments to communicate expected chatbot behavior, such as sentiment; and (c) fast, scalable development, including a CSV-driven workflow, automated testing, and integration with various devices. We implemented SafeChat in an executable framework using the open-source chatbot platform Rasa. A case study demonstrates its application in building ElectionBot-SC, a chatbot designed to safely disseminate official election information. SafeChat is being used in many domains, validating its potential, and is available at: https://github.com/ai4society/trustworthy-chatbot.

==> content/cx_removable.tex <==
\section{Can Be Removed}

% ---
\subsection{From Intro}


The foundation of a functioning democracy is its citizens' ability to participate in elections and ensure the orderly transfer of power. While Artificial Intelligence (AI) is often associated with concerns about misinformation and security during elections, chatbots offer a promising solution for improving voter participation. They provide essential information—voting dates, locations, and processes—in a user-friendly way that helps vulnerable populations, such as seniors \cite{senior-elections} and first-time voters, navigate the complexities of voting. However, concerns about generative AI's role in disseminating misinformation remain prevalent. For instance, OpenAI announced ChatGPT would defer election questions to human-curated FAQs during the 2024 elections despite its strong performance in QA settings \cite{openai-chatgpt-elections}. This emphasizes the need for specialized tools addressing election-related challenges specifically.

Researchers have assessed voting difficulty across U.S. states using metrics like the Cost of Voting Index (COVI) \cite{election-cost, COVI}, which ranks South Carolina among those with complex voting procedures due to its multi-tiered election processes covering municipal, state, and federal offices. The state's election commission oversees critical tasks such as voter registration and candidate certification. Given these complexities and the importance of empowering informed participation, tools simplifying access to reliable voting information are indispensable.

To address these challenges, we introduce \sca, a novel AI architecture designed to provide accurate, source-verified information through intent-based response generation and a provenance tracker. Unlike generative AI models prone to hallucination, \sca uses rule-based frameworks, sentiment-aware response mechanisms, and source tracking to ensure transparency and trustworthiness. As such, \sca powers \ebsc, a chatbot tool deployed to assist voters in South Carolina during the 2024 elections. This comprehensive tool was employed during South Carolina's 2024 elections at a university setting including students (first-time voters), faculty members, and staff—to explore chatbot effectiveness in addressing diverse queries related specifically to electoral matters. Our work builds on an earlier prototype deployed using 2022 data focused solely on seniors \cite{muppasani2023safe}. 

Through this work, we aim to highlight \sca’s contributions to improving domain-agnostic AI systems and demonstrate how \ebsc, powered by \sca, represents a scalable solution for addressing the evolving needs of elections and modern democracies. Beyond elections, \sca’s architecture offers a template for deploying AI systems in other sensitive domains, such as health, education, and public policy.

% ---

\subsection{Old content} - review and remove content.

\subsubsection{Domain-Agnostic Architecture}
The modular and domain-agnostic architecture of \sca is a significant asset, allowing it to be easily adapted for various applications beyond its initial deployment in South Carolina's 2024 elections. The primary customization requirement lies in the dataset pertaining to specific domains or regions. For the election domain, stakeholders can develop highly reliable local chatbots tailored to their unique informational needs by leveraging our open election FAQ dataset \cite{lakkaraju2024-electiondataset}, which compiles information from leading global democracies and U.S. states. For instance, \textit{ElectionBot-xy} where \textit{xy} is the U.S. state's identifier or a 2-letter country code.

Furthermore, this adaptability extends across multiple sectors:
\begin{itemize}
    \item In \textbf{healthcare}, the \sca architecture could build chatbots functioning as an informative tool for vaccine dissemination, providing answers to common questions about vaccination schedules, efficacy, and safety by accessing up-to-date data from health organizations.
    \item In \textbf{finance}, it can offer personalized guidance on matters such as tax filings, credit scores, or investment options by drawing from trusted financial resources like government tax portals or accredited financial advisory services.
    \item Within the realm of \textbf{education}, the architecture can assist students and educators by facilitating quick access to academic policies, course details, and resource recommendations sourced from official educational institutions.
\end{itemize}

\sca's capability to extract information from verified domain-specific sources ensures that users receive precise and trustworthy responses. This functionality not only enhances user confidence but also broadens its applicability across diverse topics and contexts, making it an invaluable tool for addressing a wide array of user inquiries across different sectors.

\subsubsection{{Planned Randomized Controlled Trial (RCT)}
\label{discussion-RCT}

While the user study provided valuable insights into the initial effectiveness and perceived accuracy of \ebsc, the randomized controlled trial (RCT) is designed to build on these findings with empirical rigor. In the RCT, participants are randomly assigned to receive responses either from the \sca engine or Google Search, allowing for a direct comparison of the two approaches in delivering voter information.

The RCT includes a pre-interaction survey (\textbf{BQ}) to establish baseline participant characteristics and a post-interaction survey (\textbf{AQ}) to evaluate the impact of using \ebsc on users’ confidence and information sufficiency. Table \ref{tab:rct_survey_questions} provides details of these survey questions.

This experimental setup aims to address the following research questions:
\begin{enumerate}
    \item Does \ebsc improve user confidence in their knowledge compared to conventional web search tools?
    \item How do users perceive the accuracy and relevance of responses provided by \ebsc relative to Google Search?
    \item What are the key factors driving user trust in a chatbot's answers within the electoral domain?
\end{enumerate}

By focusing on these outcomes, the RCT will offer a deeper understanding of the chatbot's effectiveness and potential areas for enhancement.

\begin{table}[ht]
    \centering
    \begin{tabular}{p{0.72\columnwidth}|p{0.18\columnwidth}}
        \toprule
        \textbf{Question} & \textbf{Type} \\
        \midrule
        BQ1: \textit{Are you eligible to vote in the 2024 Presidential election?} & Baseline \\[2pt]
        BQ2: \textit{If you were eligible, would you like to vote in 2024?} & Baseline \\[2pt]
        BQ3: \textit{Do you think you have all the information needed to vote?} & Baseline \\[2pt]
        BQ4: \textit{Have you ever voted before in any US election?} & Baseline \\[2pt]
        AQ1: \textit{Do you now have more relevant information to help you vote in 2024?} & Post-interaction \\[2pt]
        AQ2: \textit{Would you consider the responses you received to be accurate?} & Post-interaction \\
        \bottomrule
    \end{tabular}
    \caption{Survey Questions for the planned RCT}
    \label{tab:rct_survey_questions}
\end{table}

\subsubsection{Application Deployement}
We deploy \ebsc on Chameleon Cloud, an NSF-funded project that provides a configurable experimental environment for computer science research \cite{keahey2020lessons}. Utilizing a Kernel-based Virtual Machine (KVM), we ensure our deployment leverages the flexibility and scalability offered by Chameleon’s infrastructure. 

The application is hosted with Apache as the web server, which efficiently manages HTTP requests and ensures robust performance. To safeguard against unauthorized access, we configure stringent firewall rules, thereby securing data interactions and protecting user information. Chameleon's advanced networking features facilitate seamless integration of these security measures.

Our choice of Chameleon Cloud not only supports scalable deployment but also contributes to ongoing research efforts by providing insights into cloud-based application management and security.


